DG = FEM + flat elements, Part I: Diffusion

We establish a simple, rigorous, and easy to implement connection between the classical continuous finite element method (FEM) and the discontinuous Galerkin (DG) method for Poisson's problem. The key idea is to insert a vanishing-thickness layer of "dummy" elements along cell interfaces. By modifying the diffusion coefficient on these elements to be proportional to their thickness, we prove the FEM formulation converges to Babu\v{s}ka-Zl\'amal DG with trapezoidal edge quadrature. The scheme is trivial to implement by (i) a mesh edit that introduces degenerate interface elements and (ii) a single Jacobian threshold in an otherwise unmodified FEM code to handle the degenerate elements via the tempered finite element (TFEM) framework. We provide a rigorous derivation of the resulting TFEM-DG scheme, prove optimal $H^1$ and $L^2$ error estimates, and present numerical experiments in 2D and 3D. The method allows for simple implementation of DG in a FEM code and even adaptive element-by-element switching between FEM and DG with minimal coding effort. The framework is readily extensible, as we will demonstrate in a companion paper dedicated to evolutionary nonlinear first-order hyperbolic systems.

==> img/convergence_2D/convergence.tex <==
\begin{figure}[!ht]
    \hspace{-0.75cm}%
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={$h$},
            ylabel={$\|u - u_h\|_{L^2(\Omega)}$},
            % xmin=0.03, xmax=1.1,
            % ymin=0.00001, ymax=0.075,
            xtick={0.001, 0.01, 0.1, 1},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            ytick={0.00001, 0.0001, 0.001, 0.01, 0.1, 1},
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]

        % J_min = h ^ 2.5
        \addplot[ 
            color=blue,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.7582969458689908)
                (0.07071067811865475, 0.5094034590866163)
                (0.035355339059327376, 0.34332036612269995)
                (0.017677669529663688, 0.23354152228726752)
                (0.008838834764831844, 0.16037092022988408)
                (0.004419417382415922, 0.11098683942619227)
            };
            
        % J_min = h ^ 2.8
        \addplot[
            color=orange,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.3152230782271991)
                (0.07071067811865475, 0.17907709699744237)
                (0.035355339059327376, 0.10157731549989822)
                (0.017677669529663688, 0.05771430734790075)
                (0.008838834764831844, 0.032887352113922255)
                (0.004419417382415922, 0.018789329967769008)
            };
            
        % J_min = h ^ 3.0
        \addplot[
            color=red,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.1772786029354767)
                (0.07071067811865475, 0.09068679267652471)
                (0.035355339059327376, 0.046120516517021475)
                (0.017677669529663688, 0.023279986208761205)
                (0.008838834764831844, 0.011697287056153015)
                (0.004419417382415922, 0.005863202495668771)
            };

        % J_min = h ^ 3.5
        \addplot[
            color=teal,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.047178934018905494)
                (0.07071067811865475, 0.015855586289436632)
                (0.035355339059327376, 0.005763445823855615)
                (0.017677669529663688, 0.0021517131071037755)
                (0.008838834764831844, 0.0008009674430939619)
                (0.004419417382415922, 0.0002950210001817798)
                
            };

        % % J_min = h ^ 3.8
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1414213562373095, 0.03925094117921466)
        %         (0.07071067811865475, 0.010178615778216356)
        %         (0.035355339059327376, 0.002571746360388122)
        %         (0.017677669529663688, 0.0006555073117126156)
        %         (0.008838834764831844, 0.00017079509900469822)
        %         (0.004419417382415922, 4.5752704429384986e-05)               
        %     };

        % J_min = h ^ 4.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.04208911676731414)
                (0.07071067811865475, 0.011100619335565522)
                (0.035355339059327376, 0.0028144126190801943)
                (0.017677669529663688, 0.0007063121211337793)
                (0.008838834764831844, 0.0001767777134912739)
                (0.004419417382415922, 4.421228972314507e-05)
            };

        \addplot[color=black, mark=none] 
            coordinates {
                (0.07071067811865475, 0.0045000000000000005)
                (0.035355339059327376, 0.0011250000000000001)
                (0.017677669529663688, 0.00028125000000000003)
            };

            \node [blue, rotate=8] at (rel axis cs: 
            0.18, 0.82) { $J_{\min} = h^{2.5}$ };
            \node [orange, rotate=11] at (rel axis cs: 
            0.18, 0.68) { $J_{\min} = h^{2.8}$ };
            \node [red, rotate=15] at (rel axis cs: 
            0.18, 0.47) { $J_{\min} = h^{3.0}$ };
            \node [teal, rotate=19] at (rel axis cs: 
            0.18, 0.36) { $J_{\min} = h^{3.5}$ };
            \node [brown, rotate=28] at (rel axis cs: 
            0.24, 0.14) { $J_{\min} = h^{4.0}$ };
            \node [black, rotate=28] at (rel axis cs: 0.605,0.315) { slope 2 };

        % \legend{reference, $k=2$, $k=3$, $k=4$}

        \end{axis}
        \end{tikzpicture}%
    % \hspace{0.1cm}%
    \begin{tikzpicture}%
        \begin{axis}[
            xlabel={$h$},
            ylabel={$|u - u_h|_{H^1(\mct_h)}$},
            xtick={0.001, 0.01, 0.1, 1},
            ytick={0.1, 1, 10},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            % ymin=0.004, 
            % ymax=25,
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]
        
        % J_min = h ^ 2.5
        \addplot[
            color=blue,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 3.5654325409838354)
                (0.07071067811865475, 2.579856753607773)
                (0.035355339059327376, 1.8334127623795307)
                (0.017677669529663688, 1.2980049395419315)
                (0.008838834764831844, 0.9187055737892675)
                (0.004419417382415922, 0.6503697660911578)
            };
        
        % J_min = h ^ 2.8
        \addplot[
            color=orange,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 2.0883990964222026)
                (0.07071067811865475, 1.2172542036746299)
                (0.035355339059327376, 0.6898746937982244)
                (0.017677669529663688, 0.38840349493510246)
                (0.008838834764831844, 0.2187672071754555)
                (0.004419417382415922, 0.12353536896396343)
            };
        
        % J_min = h ^ 3.0
        \addplot[
            color=red,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 1.6547617827864474)
                (0.07071067811865475, 0.8755791618114803)
                (0.035355339059327376, 0.4475019902968222)
                (0.017677669529663688, 0.2258380176892935)
                (0.008838834764831844, 0.1133961414544369)
                (0.004419417382415922, 0.056811701832946586)
            };

        % %
        % % J_min = h ^ 3.8
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1414213562373095, 1.350644745757791)
        %         (0.07071067811865475, 0.692311694322969)
        %         (0.035355339059327376, 0.3482763345071667)
        %         (0.017677669529663688, 0.1743943760587525)
        %         (0.008838834764831844, 0.087227303584347)
        %         (0.004419417382415922, 0.043617050515471226)
        %     };
        
        % J_min = h ^ 4.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 1.3509519980313358)
                (0.07071067811865475, 0.6922036783766837)
                (0.035355339059327376, 0.34823182220049614)
                (0.017677669529663688, 0.17438273859261444)
                (0.008838834764831844, 0.0872247015373125)
                (0.004419417382415922, 0.04361651413188645)
            };

        \addplot[color=black, mark=none] 
        coordinates {
            (0.07071067811865475, 0.4596194077712559)
            (0.035355339059327376, 0.22980970388562794)
            (0.017677669529663688, 0.11490485194281397)
        };
        
        \node [blue, rotate=16] at (rel axis cs:
        0.18,0.69) { $J_{\min} = h^{2.5}$ };
        \node [orange, rotate=27] at (rel axis cs:
        0.18,0.4) { $J_{\min} = h^{2.8}$ };
        \node [red, rotate=32] at (rel axis cs:
        0.18,0.27) { $J_{\min} = h^{3.0}$ };
        \node [brown, rotate=32] at (rel axis cs:
        0.25,0.15) { $J_{\min} = h^{3.5},\,h^{4.0}$ };
        \node [black, rotate=32] at (rel axis cs:
        0.605,0.36) { slope 1 };

        \end{axis}
        \end{tikzpicture}
        \caption{Convergence behaviour of TFEM-DG in 2D for various values of $J_{\min}$ (or equivalently $D$). For $J_{\min} =h^{4.0}$ ($D=h^{-3.0}$) we obtain optimal convergence rates.}
        \label{fig:conv_2D}

    \hspace{-0.75cm}%
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={$h$},
            ylabel={$\|u - u_h\|_{L^2(\Omega)}$},
            % xmin=0.03, xmax=1.1,
            % ymin=0.00001, ymax=0.075,
            xtick={0.001, 0.01, 0.1, 1},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            ytick={0.00001, 0.0001, 0.001, 0.01, 0.1, 1},
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]

        % J_min = h ^ 4.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.04208911676731414)
                (0.07071067811865475, 0.011100619335565522)
                (0.035355339059327376, 0.0028144126190801943)
                (0.017677669529663688, 0.0007063121211337793)
                (0.008838834764831844, 0.0001767777134912739)
                (0.004419417382415922, 4.421228972314507e-05)
            };
         % J_min = h ^ 5.0
        \addplot[
            color=purple,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.05106662879847367)
                (0.07071067811865475, 0.013552364983206501)
                (0.035355339059327376, 0.003449254267460365)
                (0.017677669529663688, 0.000867413785115033)
                (0.008838834764831844, 0.0002173772131388439)
                (0.004419417382415922, 5.817507927164086e-05)
            };
        % J_min = h ^ 6.0
        \addplot[
            color=teal,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.052177081829180794)
                (0.07071067811865475, 0.013701884864903788)
                (0.035355339059327376, 0.0034685183650109484)
                (0.017677669529663688, 0.0008698336797826946)
                (0.008838834764831844, 0.000220629475412624)
                (0.004419417382415922, 0.0003790196744962833)
            };

        % J_min = h ^ 7.0
        \addplot[
            color=violet,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 0.0522897323688261)
                (0.07071067811865475, 0.013709413543225472)
                (0.035355339059327376, 0.003469102838909529)
                (0.017677669529663688, 0.0008713972782145685)
                (0.008838834764831844, 0.0009654656059442646)
                (0.004419417382415922, 0.02220425552441099)
            };

        \addplot[color=black, mark=none] 
            coordinates {
                (0.1414213562373095, 0.0045000000000000005)
                (0.07071067811865475, 0.0011250000000000001)
                (0.035355339059327376, 0.00028125000000000003)
            };

            % \node [blue, rotate=8] at (rel axis cs: 
            % 0.18, 0.82) { $J_{\min} = h^{2.5}$ };
            % \node [orange, rotate=11] at (rel axis cs: 
            % 0.18, 0.68) { $J_{\min} = h^{2.8}$ };
            % \node [red, rotate=15] at (rel axis cs: 
            % 0.18, 0.47) { $J_{\min} = h^{3.0}$ };
            \node [brown, rotate=37] at (rel axis cs: 
            0.48, 0.4) { $J_{\min} = h^{4.0}$ };
            \node [purple, rotate=36] at (rel axis cs: 
            0.24, 0.16) { $J_{\min} = h^{5.0}$ };
            \node [teal, rotate=0] at (rel axis cs: 
            0.14, 0.4) { $J_{\min} = h^{6.0}$ };
            \node [violet, rotate=0] at (rel axis cs: 
            0.24, 0.8) { $J_{\min} = h^{7.0}$ };
            \node [black, rotate=39] at (rel axis cs: 0.770,0.42) { slope 2 };

        % \legend{reference, $k=2$, $k=3$, $k=4$}

        \end{axis}
        \end{tikzpicture}%
    % \hspace{0.1cm}%
    \begin{tikzpicture}%
        \begin{axis}[
            xlabel={$h$},
            ylabel={$|u - u_h|_{H^1(\mct_h)}$},
            xtick={0.001, 0.01, 0.1, 1},
            ytick={0.1, 1, 10},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            % ymin=0.004, 
            % ymax=25,
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]
        
        % J_min = h ^ 4.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 1.3509519980313358)
                (0.07071067811865475, 0.6922036783766837)
                (0.035355339059327376, 0.34823182220049614)
                (0.017677669529663688, 0.17438273859261444)
                (0.008838834764831844, 0.0872247015373125)
                (0.004419417382415922, 0.04361651413188645)
            };

        % % J_min = h ^ 5.0
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1414213562373095, 1.3576827778633953)
        %         (0.07071067811865475, 0.6930949338360601)
        %         (0.035355339059327376, 0.34834570829198963)
        %         (0.017677669529663688, 0.17439711280583078)
        %         (0.008838834764831844, 0.08722650648269878)
        %         (0.004419417382415922, 0.04361676366127306)
        %     };

        % % J_min = h ^ 6.0
        % \addplot[
        %     color=teal,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1414213562373095, 1.3587734320182452)
        %         (0.07071067811865475, 0.6931681255525899)
        %         (0.035355339059327376, 0.34835041339986456)
        %         (0.017677669529663688, 0.17439741052531135)
        %         (0.008838834764831844, 0.08722654018597945)
        %         (0.004419417382415922, 0.04371864343444853)
        %     };

        % J_min = h ^ 7.0
        \addplot[
            color=violet,
            mark=*,
            ]
            coordinates {
                (0.1414213562373095, 1.3588866652885918)
                (0.07071067811865475, 0.6931718566558817)
                (0.035355339059327376, 0.34835053219028195)
                (0.017677669529663688, 0.17439741915819695)
                (0.008838834764831844, 0.08744984718068946)
                (0.004419417382415922, 0.2931769850554141)
            };

        \addplot[color=black, mark=none] 
        coordinates {
            (0.1414213562373095, 0.4596194077712559)
            (0.07071067811865475, 0.22980970388562794)
            (0.035355339059327376, 0.11490485194281397)
        };
        
        % \node [blue, rotate=16] at (rel axis cs:
        % 0.18,0.69) { $J_{\min} = h^{2.5}$ };
        % \node [orange, rotate=27] at (rel axis cs:
        % 0.18,0.4) { $J_{\min} = h^{2.8}$ };
        % \node [red, rotate=32] at (rel axis cs:
        % 0.18,0.27) { $J_{\min} = h^{3.0}$ };
        \node [brown, rotate=39] at (rel axis cs:
        0.35,0.27) { $J_{\min} = h^{4.0},\,h^{5.0},\,h^{6.0}$ };
        \node [violet, rotate=0] at (rel axis cs:
        0.25,0.5) { $J_{\min} = h^{7.0}$ };
        \node [black, rotate=39] at (rel axis cs:
        0.775,0.45) { slope 1 };

        \end{axis}
        \end{tikzpicture}
        \caption{Convergence behavior for values of $J_{\min}$ that are lower than $h^{4.0}$. The order is preserved, as the theory states. However, some problems arise when the value of $J_{\min}$ nears machine precision.}
        \label{fig:conv_2D_2}
\end{figure}

==> img/convergence_3D/convergence_3D.tex <==
\begin{figure}[!ht]
    \hspace{-0.75cm}%
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={$h$},
            ylabel={$\|u - u_h\|_{L^2(\Omega)}$},
            ymax=2,
            xtick={0.001, 0.01, 0.1, 1},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            ytick={0.00001, 0.0001, 0.001, 0.01, 0.1, 1},
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]

        % J_min = h ^ 3.5
        \addplot[ 
            color=blue,
            mark=*,
            ]
            coordinates {
                (0.1, 0.5444875453447039)
                (0.08333333333333333, 0.4862247149837414)
                (0.06666666666666667, 0.4388884653365839)
                (0.05, 0.34804947853748874)
                (0.04, 0.3133799878074649)
                (0.03225806451612903, 0.27568971092386807)
                (0.025, 0.24084237871827643)
            };
            
        % J_min = h ^ 3.8
        \addplot[
            color=orange,
            mark=*,
            ]
            coordinates {
                (0.1, 0.20847416744231645)
                (0.08333333333333333, 0.18101692353267484)
                (0.06666666666666667, 0.15696298451001386)
                (0.05, 0.11792774933903603)
                (0.04, 0.10134219561908844)
                (0.03225806451612903, 0.08499930519757048)
                (0.025, 0.06997111562701182)
            };
            
        % J_min = h ^ 4.0
        \addplot[
            color=red,
            mark=*,
            ]
            coordinates {
                (0.1, 0.10915459321666536)
                (0.08333333333333333, 0.09343232078478675)
                (0.06666666666666667, 0.0793236848746143)
                (0.05, 0.057651994883991496)
                (0.04, 0.04827334351133571)
                (0.03225806451612903, 0.03935310436033498)
                (0.025, 0.031247703061875944)
            };

        % J_min = h ^ 4.5
        \addplot[
            color=teal,
            mark=*,
            ]
            coordinates {
                (0.1, 0.02832445318073074) 
                (0.08333333333333333, 0.02029085883591245) 
                (0.06666666666666667, 0.014160503262172169) 
                (0.05, 0.008585033789524944) 
                (0.04, 0.006303393227507592) 
                (0.03225806451612903, 0.0046527588142112105) 
                (0.025, 0.00333218201643245)
            };

        % % J_min = h ^ 4.8
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1, 0.032855134584366355)
        %         (0.08333333333333333, 0.02256014916701544)
        %         (0.06666666666666667, 0.014559452326031893)
        %         (0.05, 0.008190761804665894)
        %         (0.04, 0.005151523587776253)
        %         (0.03225806451612903, 0.0033114548554792275)
        %         (0.025, 0.0019530995613257533) 
        %     };

        % J_min = h ^ 5.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1, 0.03732797661597756)
                (0.08333333333333333, 0.025927722289159016)
                (0.06666666666666667, 0.017010682385539013)
                (0.05, 0.009699537431328821)
                (0.04, 0.006205256197923063)
                (0.03225806451612903, 0.00403660324006052)
                (0.025, 0.002418616747956514)
            };

        \addplot[color=black, mark=none] 
            coordinates {
                (0.07071067811865475, 0.01)
                (0.035355339059327376, 0.0025)
            };

            \node [blue, rotate=4] at (rel axis cs: 
            0.18, 0.78) { $J_{\min} = h^{3.5}$ };
            \node [orange, rotate=6] at (rel axis cs: 
            0.18, 0.62) { $J_{\min} = h^{3.8}$ };
            \node [red, rotate=9] at (rel axis cs: 
            0.18, 0.39) { $J_{\min} = h^{4.0}$ };
            \node [teal, rotate=11] at (rel axis cs: 
            0.18, 0.22) { $J_{\min} = h^{4.5}$ };
            \node [brown, rotate=19] at (rel axis cs: 
            0.48, 0.33) { $J_{\min} = h^{5.0}$ };
            \node [black, rotate=20] at (rel axis cs: 0.52,0.14) { slope 2 };

        % \legend{reference, $k=2$, $k=3$, $k=4$}

        \end{axis}
        \end{tikzpicture}%
    % \hspace{0.1cm}%
    \begin{tikzpicture}%
        \begin{axis}[
            xlabel={$h$},
            ylabel={$|u - u_h|_{H^1(\mct_h)}$},
            xtick={0.001, 0.01, 0.1, 1},
            ytick={0.1, 1, 10},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            ymax=6,
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]
        
        % J_min = h ^ 3.5
        \addplot[
            color=blue,
            mark=*,
            ]
            coordinates {
                (0.1, 3.676424089804899)
                (0.08333333333333333, 3.472578884381604)
                (0.06666666666666667, 3.178016703598315)
                (0.05, 2.694870726612171)
                (0.04, 2.474364926356051)
                (0.03225806451612903, 2.219845426124182)
                (0.025, 1.9745023306372869)
            };
        
        % J_min = h ^ 3.8
        \addplot[
            color=orange,
            mark=*,
            ]
            coordinates {
                (0.1, 2.1164579514793265)
                (0.08333333333333333, 1.8934201016548724)
                (0.06666666666666667, 1.6187453083732435)
                (0.05, 1.2677576854254216)
                (0.04, 1.0787438804019625)
                (0.03225806451612903, 0.9040387359254932)
                (0.025, 0.7387201432387377)
            };
        
        % J_min = h ^ 4.0
        \addplot[
            color=red,
            mark=*,
            ]
            coordinates {
                (0.1, 1.6802297844639997)
                (0.08333333333333333, 1.4578344732676691)
                (0.06666666666666667, 1.203400778998302)
                (0.05, 0.9134237614155067)
                (0.04, 0.7474528113188496)
                (0.03225806451612903, 0.6077355238626339)
                (0.025, 0.47660150059259043) 
            };

        % % J_min = h ^ 4.5
        % \addplot[
        %     color=teal,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1, 1.4252885447285346) 
        %         (0.08333333333333333, 1.2106334904789513) 
        %         (0.06666666666666667, 0.9798392186283703) 
        %         (0.05, 0.7413317954420056) 
        %         (0.04, 0.5963656717942055) 
        %         (0.03225806451612903, 0.4823174878641951) 
        %         (0.025, 0.37428439786311374)
        %     };

        % % J_min = h ^ 4.8
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %            (0.1, 1.4280654203235708) 
        %            (0.08333333333333333, 1.210823989935079) 
        %            (0.06666666666666667, 0.9778246723586813) 
        %            (0.05, 0.739229392201489) 
        %            (0.04, 0.5942567147870148) 
        %            (0.03225806451612903, 0.4806510611625591) 
        %            (0.025, 0.3729814691927163)       
        %     };
        
        % J_min = h ^ 5.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
               (0.1, 1.436433032480107)
               (0.08333333333333333, 1.2163798307893394)
               (0.06666666666666667, 0.9807396795472509)
               (0.05, 0.7404701057360122)
               (0.04, 0.5949015386142209)
               (0.03225806451612903, 0.4810016055429853)
               (0.025, 0.37313426058382065) 
            };

        \addplot[color=black, mark=none] 
        coordinates {
            (0.09, 0.8)
            (0.045, 0.4)
        };
        
        \node [blue, rotate=10] at (rel axis cs:
        0.18,0.72) { $J_{\min} = h^{3.5}$ };
        \node [orange, rotate=19] at (rel axis cs:
        0.18,0.42) { $J_{\min} = h^{3.8}$ };
        \node [red, rotate=21] at (rel axis cs:
        0.18,0.28) { $J_{\min} = h^{4.0}$ };
        \node [brown, rotate=24] at (rel axis cs:
        0.25,0.13) { $J_{\min} = h^{4.5},\,h^{5.0}$ };
        \node [black, rotate=24] at (rel axis cs:
        0.65,0.16) { slope 1 };

        \end{axis}
        \end{tikzpicture}
        \caption{Convergence behavior of TFEM-DG in 3D for various values of $J_{\min}$ (or equivalently $D$). For $J_{\min} =h^{5.0}$ ($D=h^{-3.0}$) we obtain optimal convergence rates.}
        \label{fig:conv_3D}

    \hspace{-0.75cm}%
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={$h$},
            ylabel={$\|u - u_h\|_{L^2(\Omega)}$},
            % xmin=0.03, xmax=1.1,
            % ymin=0.00001, ymax=0.075,
            xtick={0.001, 0.01, 0.1, 1},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            ytick={0.00001, 0.0001, 0.001, 0.01, 0.1, 1},
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]

        % J_min = h ^ 5.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1, 0.03732797661597756)
                (0.08333333333333333, 0.025927722289159016)
                (0.06666666666666667, 0.017010682385539013)
                (0.05, 0.009699537431328821)
                (0.04, 0.006205256197923063)
                (0.03225806451612903, 0.00403660324006052)
                (0.025, 0.002418616747956514) 
            };
        %  % J_min = h ^ 6.0
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1, 0.04560875575025788)
        %         (0.08333333333333333, 0.03183669168368628)
        %         (0.06666666666666667, 0.02103292688064683)
        %         (0.05, 0.011917423758554575)
        %         (0.04, 0.007674868831801262)
        %         (0.03225806451612903, 0.004994270599571774)
        %         (0.025, 0.0030021850889776144) 
        %     };
        % J_min = h ^ 7.0
        \addplot[
            color=teal,
            mark=*,
            ]
            coordinates {
                (0.1, 0.0464950173508029)
                (0.08333333333333333, 0.03236670914395782)
                (0.06666666666666667, 0.02132259739484741)
                (0.05, 0.012036912111596377)
                (0.04, 0.007738414438898282)
                (0.03225806451612903, 0.005027716844490401)
                (0.025, 0.003018023277165288)
            };

        % J_min = h ^ 10.0
        \addplot[
            color=violet,
            mark=*,
            ]
            coordinates {
                (0.1, 0.046593865439080735) 
                (0.08333333333333333, 0.03241508577418363)
                (0.06666666666666667, 0.02134337602037686)
                (0.05, 0.01204334209935446)
                (0.04, 0.007742905122999807)
                (0.03225806451612903, 0.005046038227094528)
                (0.025, 0.0031589381820582973)
            };

        \addplot[color=black, mark=none] 
            coordinates {
                (0.09, 0.015)
                (0.045, 0.00375)
            };

            % \node [blue, rotate=8] at (rel axis cs: 
            % 0.18, 0.82) { $J_{\min} = h^{2.5}$ };
            % \node [orange, rotate=11] at (rel axis cs: 
            % 0.18, 0.68) { $J_{\min} = h^{2.8}$ };
            % \node [red, rotate=15] at (rel axis cs: 
            % 0.18, 0.47) { $J_{\min} = h^{3.0}$ };
            \node [brown, rotate=37] at (rel axis cs: 
            0.32, 0.22) { $J_{\min} = h^{5.0},\,h^{6.0}$ };
            % \node [purple, rotate=36] at (rel axis cs: 
            % 0.24, 0.16) { $J_{\min} = h^{6.0}$ };
            \node [teal, rotate=36] at (rel axis cs: 
            0.18, 0.31) { $J_{\min} = h^{7.0}$ };
            \node [violet, rotate=37] at (rel axis cs: 
            0.44, 0.55) { $J_{\min} = h^{10.0}$ };
            \node [black, rotate=39] at (rel axis cs: 0.66,0.35) { slope 2 };

        % \legend{reference, $k=2$, $k=3$, $k=4$}

        \end{axis}
        \end{tikzpicture}%
    % \hspace{0.1cm}%
    \begin{tikzpicture}%
        \begin{axis}[
            xlabel={$h$},
            ylabel={$|u - u_h|_{H^1(\mct_h)}$},
            xtick={0.001, 0.01, 0.1, 1},
            ytick={0.1, 1, 10},
            xticklabel style={above, yshift=1ex, xshift=1ex},
            % ymin=0.004, 
            % ymax=25,
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            xmode=log,
            ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.0)},anchor=north},
            y label style={at={(axis description cs:0.2,0.85)},rotate=-90,anchor=south},
        ]
        
        % J_min = h ^ 5.0
        \addplot[
            color=brown,
            mark=*,
            ]
            coordinates {
                (0.1, 1.436433032480107)
                (0.08333333333333333, 1.2163798307893394)
                (0.06666666666666667, 0.9807396795472509)
                (0.05, 0.7404701057360122)
                (0.04, 0.5949015386142209)
                (0.03225806451612903, 0.4810016055429853)
                (0.025, 0.37313426058382065)
            };

        % % J_min = h ^ 6.0
        % \addplot[
        %     color=purple,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1, 1.457675056234071)
        %         (0.08333333333333333, 1.2294517356883938)
        %         (0.06666666666666667, 0.9872550894395574)
        %         (0.05, 0.743030532662518)
        %         (0.04, 0.5962126569865174)
        %         (0.03225806451612903, 0.48168585497311633)
        %         (0.025, 0.3734405219927489)
        %     };

        % % J_min = h ^ 7.0
        % \addplot[
        %     color=teal,
        %     mark=*,
        %     ]
        %     coordinates {
        %         (0.1, 1.4603836903007779)
        %         (0.08333333333333333, 1.230819904548234)
        %         (0.06666666666666667, 0.9877996779207909)
        %         (0.05, 0.7431901998430103)
        %         (0.04, 0.5962785011497673)
        %         (0.03225806451612903, 0.48171353598409083)
        %         (0.025, 0.37345022931434174)
        %     };

        % J_min = h ^ 10.0
        \addplot[
            color=violet,
            mark=*,
            ]
            coordinates {
                (0.1, 1.4606911277781078)
                (0.08333333333333333, 1.23094636175716)
                (0.06666666666666667, 0.9878390937430422)
                (0.05, 0.743198685728631)
                (0.04, 0.5962812678078255)
                (0.03225806451612903, 0.48171455654573825)
                (0.025, 0.373457344835768)
            };

        \addplot[color=black, mark=none] 
        coordinates {
            (0.09, 0.9)
            (0.045, 0.45)
        };
        
        % \node [blue, rotate=16] at (rel axis cs:
        % 0.18,0.69) { $J_{\min} = h^{2.5}$ };
        % \node [orange, rotate=27] at (rel axis cs:
        % 0.18,0.4) { $J_{\min} = h^{2.8}$ };
        % \node [red, rotate=32] at (rel axis cs:
        % 0.18,0.27) { $J_{\min} = h^{3.0}$ };
        \node [brown, rotate=39] at (rel axis cs:
        0.35,0.27) { $J_{\min} = h^{5.0},\,h^{6.0},\,h^{7.0}$ };
        \node [violet, rotate=39] at (rel axis cs:
        0.3,0.4) { $J_{\min} = h^{10.0}$ };
        \node [black, rotate=39] at (rel axis cs:
        0.7,0.37) { slope 1 };

        \end{axis}
        \end{tikzpicture}
        \caption{Convergence behavior for values of $J_{\min}$ that are lower than $h^{5.0}$. The order is preserved, as the theory states.}        
        \label{fig:conv_3D_2}
\end{figure}

==> img/example_1D/numerical_experiment_1D_plot.tex <==

\begin{figure}[!ht]
    \hspace{-0.4cm}%
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={$x$},
            ylabel={$D = h^{-2}$},
            % xmin=0.03, xmax=1.1,
            % ymin=0.00001, ymax=0.075,
            xtick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
            xticklabel style={below, yshift=0ex, xshift=0ex},
            ytick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            % xmode=log,
            % ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.05)},anchor=north},
            y label style={at={(axis description cs:0.85,0.85)},rotate=-90,anchor=south},
            domain=0.0:1.0
        ]

        \addplot[
            smooth,
            color=red,
            style=dashed,
        ] {4*x*(1-x)};

        \addplot[
        color=blue,
        ]
        coordinates {
            (0.0, 0.04000000000000001)
            (0.1, 0.4000000000000001)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.1, 0.43200000000000005)
            (0.2, 0.7120000000000001)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.2, 0.736)
            (0.30000000000000004, 0.9360000000000002)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.30000000000000004, 0.952)
            (0.4, 1.072)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.4, 1.08)
            (0.5, 1.12)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.5, 1.12)
            (0.6000000000000001, 1.08)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.6000000000000001, 1.072)
            (0.7000000000000001, 0.952)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.7000000000000001, 0.9360000000000002)
            (0.8, 0.736)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.8, 0.7120000000000001)
            (0.9, 0.43200000000000005)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.9, 0.4000000000000001)
            (1.0, 0.04000000000000001)
        };

        \addplot[
        color=black,
        ]
        coordinates {
            (0.1, 0.4000000000000001)
            (0.1, 0.43200000000000005)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.2, 0.7120000000000001)
            (0.2, 0.736)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.30000000000000004, 0.9360000000000002)
            (0.30000000000000004, 0.952)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.4, 1.072)
            (0.4, 1.08)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.5, 1.12)
            (0.5, 1.12)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.6000000000000001, 1.08)
            (0.6000000000000001, 1.072)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.7000000000000001, 0.952)
            (0.7000000000000001, 0.9360000000000002)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.8, 0.736)
            (0.8, 0.7120000000000001)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.9, 0.43200000000000005)
            (0.9, 0.4000000000000001)
        };

        \node [blue, rotate=0] at (rel axis cs:
        0.75, 0.8) { $u_h(x)$ };
        \node [red, rotate=0] at (rel axis cs:
        0.65, 0.6) { $u(x)$ };
            
        \end{axis}
    \end{tikzpicture}
    \hspace{0.1cm}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={$x$},
            ylabel={$D = h^{-3}$},
            % xmin=0.03, xmax=1.1,
            % ymin=0.00001, ymax=0.075,
            xtick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
            xticklabel style={below, yshift=0ex, xshift=0ex},
            ytick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
            legend pos=north west,
            ymajorgrids=true,
            grid=none,
            % xmode=log,
            % ymode=log,
            width=0.56\textwidth,
            height=0.47\textwidth,
            x label style={at={(axis description cs:0.5,-0.05)},anchor=north},
            y label style={at={(axis description cs:0.85,0.85)},rotate=-90,anchor=south},
            domain=0.0:1.0
        ]

        \addplot[
            smooth,
            color=red,
            style=dashed,
        ] {4*x*(1-x)};

        \addplot[
        color=blue,
        ]
        coordinates {
            (0.0, 0.004000000000000002)
            (0.1, 0.3640000000000001)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.1, 0.36720000000000014)
            (0.2, 0.6472000000000002)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.2, 0.6496000000000002)
            (0.30000000000000004, 0.8496000000000002)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.30000000000000004, 0.8512000000000004)
            (0.4, 0.9712000000000004)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.4, 0.9720000000000004)
            (0.5, 1.0120000000000005)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.5, 1.0120000000000005)
            (0.6000000000000001, 0.9720000000000004)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.6000000000000001, 0.9712000000000004)
            (0.7000000000000001, 0.8512000000000004)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.7000000000000001, 0.8496000000000002)
            (0.8, 0.6496000000000002)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.8, 0.6472000000000002)
            (0.9, 0.36720000000000014)
        };
        
        \addplot[
        color=blue,
        ]
        coordinates {
            (0.9, 0.3640000000000001)
            (1.0, 0.004000000000000002)
        };

        \addplot[ 
        color=black,
        ]
        coordinates {
            (0.1, 0.3640000000000001) 
            (0.1, 0.36720000000000014)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.2, 0.6472000000000002)
            (0.2, 0.6496000000000002)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.30000000000000004, 0.8496000000000002)
            (0.30000000000000004, 0.8512000000000004)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.4, 0.9712000000000004)
            (0.4, 0.9720000000000004)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.5, 1.0120000000000005)
            (0.5, 1.0120000000000005)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.6000000000000001, 0.9720000000000004)
            (0.6000000000000001, 0.9712000000000004)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.7000000000000001, 0.8512000000000004)
            (0.7000000000000001, 0.8496000000000002)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.8, 0.6496000000000002)
            (0.8, 0.6472000000000002)
        };
        
        \addplot[
        color=black,
        ]
        coordinates {
            (0.9, 0.36720000000000014)
            (0.9, 0.3640000000000001)
        };

        \node [blue, rotate=0] at (rel axis cs:
        0.75, 0.8) { $u_h(x)$ };
        \node [red, rotate=0] at (rel axis cs:
        0.65, 0.6) { $u(x)$ };
            
        \end{axis}
    \end{tikzpicture}
    \caption{TFEM-DG solution of the problem $-u^{\prime\prime}=4$ on $[0,1]$. 10 elements, $D=h^{-2}$ (left), $D=h^{-3}$ (right).}
    \label{fig:1D}
\end{figure}

